WDNet: Watermark-Decomposition Network for Visible Watermark Removal

Visible watermarks are widely-used in images to protect copyright ownership. Analyzing watermark removal helps to reinforce the anti-attack techniques in an adversarial way. Current removal methods normally leverage image-to-image translation techniques. Nevertheless, the uncertainty of the size, shape, color and transparency of the watermarks set a huge barrier for these methods. To combat this, we combine traditional watermarked image decomposition into a two-stage generator, called Watermark-Decomposition Network (WDNet), where the first stage predicts a rough decomposition from the whole watermarked image and the second stage specifically centers on the watermarked area to refine the removal results. The decomposition formulation enables WDNet to separate watermarks from the images rather than simply removing them. We further show that these separated watermarks can serve as extra nutrients for building a larger training dataset and further improving removal performance. Besides, we construct a large-scale dataset named CLWD, which mainly contains colored watermarks, to fill the vacuum of colored watermark removal dataset. Extensive experiments on the public gray-scale dataset LVW and CLWD consistently show that the proposed WDNet outperforms the state-of-the-art approaches both in accuracy and efficiency. The code and CLWD dataset are publicly available at https://github.com/MRUIL/WDNet.

==> images/fig_ablation_result_CLWD.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{images/ablation_result_CLWD.pdf}
\caption{Qualitative ablation comparisons on CLWD dataset. }
%\caption{Qualitative comparisons with state-of-the-art on some images from LVW and CLWD. The watermarks is the results of WDNet.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
\label{fig:ablation_study_clwd}
\centering
\end{figure*}

==> images/fig_ablation_result_LVW.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{images/ablation_result_LVW.pdf}
\caption{Qualitative ablation comparisons on LVW dataset. }
%\caption{Qualitative comparisons with state-of-the-art on some images from LVW and CLWD. The watermarks is the results of WDNet.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
\label{fig:ablation_study_lvw}
\centering
\end{figure*}

==> images/fig_result_sub_CLWD.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=\linewidth]{images/result_img_supplementary_CLWD.pdf}
\caption{Qualitative comparisons with Li~\etal~\cite{Li2019TowardsPV} on CLWD dataset. The watermarks in the last column are obtained by our WDNet.  }
%\caption{Qualitative comparisons with state-of-the-art on some images from LVW and CLWD. The watermarks is the results of WDNet.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
\label{fig:figresult_sub_clwd}
\centering
\end{figure*}

==> images/fig_time_rmse_clwd.tex <==
\begin{figure}
%\setlength{\abovedisplayskip}{3pt}
%\setlength{\belowdisplayskip}{3pt}
\centering
\includegraphics[width=\linewidth]{images/time_rmse_CLWD.pdf}
\caption{WDNet achieves state-of-the-art performance while higher operating efficiency on the CLWD dataset. We plot the trade-off between efficiency and $\mathrm{RMSE}_{w}$.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
%\setlength{\belowcaptionskip}{-5pt}
\label{fig:time_rmse}
\centering
\end{figure}

==> images/tab_function_analysis_2.tex <==
\begin{table*}[]

\small
\renewcommand\arraystretch{1.2}
\begin{center}
\resizebox{\linewidth}{12mm}{
\begin{tabular}{cc|c|c|c|c|c|c|c}
\hline
        & \multicolumn{4}{c|}{LVW} & \multicolumn{4}{c}{CLWD} \\ \hline
\multicolumn{1}{c|}{Function} & $PSNR$ & $SSIM$   & $RMSE_{w}$      & $RMSE_{all}$      & $PSNR$   & $SSIM$    & $RMSE_{w}$      & $RMSE_{all}$  \\ \hline
\multicolumn{1}{c|}{No mask+Direct}    & 17.10    & 0.9843       & 15.72     & 3.68    & 34.88      & 0.9763        & 25.42     & 4.71    \\ \hline
\multicolumn{1}{c|}{Detecting mask+Direct}    & 41.91   & 0.9966       & 13.84     & 2.21       & 39.98   & 0.9930        & 19.05     & 2.72   \\ \hline
\multicolumn{1}{c|}{Detecting mask+Direct+RefineNet}    & 42.19    & \bf{0.9967}       & 12.81     & 2.13    & 39.96      & 0.9931        & \bf{18.36}     & 2.92    \\ \hline
\multicolumn{1}{c|}{Detecting mask+Indirect+RefineNet}    & \bf{42.33}   & 0.9966       & \bf{12.38}     & \bf{2.10}       & \bf{40.23}   & \bf{0.9934}        & 18.4     & \bf{2.65}   \\ \hline
\end{tabular}}
\end{center}
\caption{Ablation results on both the LVW and the CLWD datasets.}
\label{tab:function_analysis}
\end{table*}

==> supplementary_images/fig_sup_ablation.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{supplementary_images/sup_ablation_result.pdf}
\caption{Qualitative ablation comparisons on LVW (the first row) and CLWD (the second row) datasets. }
%\caption{Qualitative comparisons with state-of-the-art on some images from LVW and CLWD. The watermarks is the results of WDNet.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
\label{fig:sup_ablation_study_clwd}
\centering
\end{figure*}

==> supplementary_images/fig_sup_state_of_the_art.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{supplementary_images/sup_result_state_of_the_art.pdf}
\caption{Qualitative comparisons with some other methods on some images from CLWD. The watermarks in the last column are obtained by our WDNet.}
%\caption{Qualitative comparisons with state-of-the-art on some images from LVW and CLWD. The watermarks is the results of WDNet.}
%\caption{Trade-off between efficiency and accuracy for some existing methods and the proposed super-BPD. Based on the region F-measure~\cite{pont2016supervised}, super-BPD achieves competing performance while being near real-time on the PASCAL Context Dataset~\cite{mottaghi2014role}.}
\label{fig:supp_compare_results}
\centering
\end{figure*}

==> supplementary_images/tab_sup_loss_weight.tex <==
\begin{table}[!h]
\small
\renewcommand\arraystretch{1.2}
\begin{center}
\begin{tabular}{c|c|c|c|c}
\toprule[1pt]
$\lambda_1$        &1   & 10    &50        & 100\\ \hline
$\mathrm{RMSE}_w$        & 19.58 & 18.36  & \bf{17.49} & 17.92\\  
\midrule[1pt]
$\lambda_2$        &1e-3   & 1e-2    &1e-1        & 1\\ \hline
$\mathrm{RMSE}_w$        & 19.01 & \bf{17.49}  &18.09  &18.23 \\  
\midrule[1pt]
$\lambda_3$        &1   & 10    &50        & 100\\ \hline
$\mathrm{RMSE}_w$        & 18.33 & \bf{17.49}  & 18.17 & 18.42\\  
\midrule[1pt]
$\lambda_4$        &1   & 10    &50        & 100\\ \hline
$\mathrm{RMSE}_w$        & 18.49 & \bf{17.49}  & 18.64 &19.82 \\  
\bottomrule[1pt]
\end{tabular}
\end{center}
%\vspace{-1mm}
\caption{Effects of four Loss weights on the performance $\mathrm{RMSE}_w$.}
\label{tab:sup_influenceoflossweights}
%\vspace{-4mm}
\end{table}

==> tab_function_analysis.tex <==
\begin{table*}[]
\small
\renewcommand\arraystretch{1.2}
\begin{center}
\begin{tabular}{c|c|c|c|c|c}
\toprule[1pt]
Dataset &Models & $\mathrm{PSNR}$ & $\mathrm{SSIM}$ & $\mathrm{RMSE}_{w}$ & $\mathrm{RMSE}_{all}$\\
\bottomrule[1pt]
%\multicolumn{2}{c|}{VI} & \multirow{2}{*}{Time (s)} \\ \cline{3-12}
%                                      && ODS         & OIS        & ODS        & OIS        & ODS        & OIS        & ODS         & OIS        & ODS         & OIS &\\\midrule[1pt]
\multirow{4}{*}{LVW} &no mask$+$direct           & 37.10      & 0.9843       & 15.72        & 3.68\\
&mask$+$direct           & 41.91      & 0.9966       & 13.84        & 2.21\\
&mask$+$direct$+$direct           & 42.19      & \bf{0.9967}       & 12.81        & 2.13\\
&mask$+$indirect$+$direct           & \bf{42.33}      & 0.9966       & \bf{12.38}        & \bf{2.10}\\ 
\bottomrule[1pt] 
\multirow{4}{*}{CLWD} &no mask$+$direct           & 34.88      & 0.9763       & 25.42        & 4.71\\
&mask$+$direct           & 39.98      & 0.9930       & 19.05        & 2.72\\
&mask$+$direct$+$direct           & 39.96      & 0.9931       & \bf{18.36}        & 2.92\\
&mask$+$indirect$+$direct           & \bf{40.23}      & \bf{0.9934}       & 18.4        & \bf{2.65}\\ 
\bottomrule[1pt] 
\end{tabular}
\end{center}
%\vspace{-1mm}
%\caption{Quantitative evaluation on the PASCAL Context and BSDS500 dataset.  Super-BPD achieves the state-of-the-art performance among real-time methods ($2^{\text{nd}}$ row) and remains competitive against non-real-time methods. GT* is the rough annotation following~\cite{liu2018deep}.}
\caption{Ablation results on both the LVW and the CLWD datasets.}
\label{tab:function_analysis_1}
\end{table*}

==> tab_state_of_art.tex <==
\begin{table*}[]
\small
\renewcommand\arraystretch{1.2}
\begin{center}
\begin{tabular}{c|c|c|c|c|c}
\toprule[1pt]
Dataset &Method & $\mathrm{PSNR}$ & $\mathrm{SSIM}$ & $\mathrm{RMSE}_{w}$ & $\mathrm{RMSE}_{all}$\\
\bottomrule[1pt]
%\multicolumn{2}{c|}{VI} & \multirow{2}{*}{Time (s)} \\ \cline{3-12}
%                                      && ODS         & OIS        & ODS        & OIS        & ODS        & OIS        & ODS         & OIS        & ODS         & OIS &\\\midrule[1pt]

%&Cheng \etal~\cite{Cheng2018LargeScaleVW}           & -      & -       & -        & -\\
\multirow{2}{*}{LVW} &Li \etal~\cite{Li2019TowardsPV}      & 34.01      & 0.9700       & 26.24        & 5.34\\
&Ours           & \bf{42.33}      & \bf{0.9966}       & \bf{12.38}        & \bf{2.10}\\ 
\bottomrule[1pt]
%&Cheng \etal~\cite{Cheng2018LargeScaleVW}           & -      & -       & -        & -\\
\multirow{2}{*}{CLWD} &Li \etal~\cite{Li2019TowardsPV}           & 32.62      & 0.9664       & 34.16        & 6.07\\
&Ours           & \bf{40.23}      & \bf{0.9934}       & \bf{18.4}        & \bf{2.65}\\ 
\bottomrule[1pt] 
\end{tabular}
\end{center}
%\vspace{-1mm}
%\caption{Quantitative evaluation on the PASCAL Context and BSDS500 dataset.  Super-BPD achieves the state-of-the-art performance among real-time methods ($2^{\text{nd}}$ row) and remains competitive against non-real-time methods. GT* is the rough annotation following~\cite{liu2018deep}.}
\caption{Comparisons with state-of-the-art method on LVW and CLWD dataset.}
\label{tab:state_of_art_1}
\end{table*}
